On the second largest component of random hyperbolic graphs

We show that in the random hyperbolic graph model as formalized by Gugelmann et al. in the most interesting range of $\frac12 < \alpha < 1$ the size of the second largest component is $\Theta((\log n)^{1/(1-\alpha)})$, thus answering a question of Bode et al. We also show that for $\alpha=\frac12$ with constant probability the corresponding size is $\Theta(\log n)$, whereas for $\alpha=1$ it is $\Omega(n^{b})$ for some $b > 0$.

==> secDiscussion.tex <==
\section{Boundary cases of $\alpha$}\label{sec:boundary}
%
As noted in the introduction, for the hyperbolic random graph model, 
  the interesting range of the parameter is when $\frac12\leq\alpha\leq 1$.
In this section we investigate the size of the second largest component
  when $\alpha$ takes the values $\frac12$ or $1$.

\subsection{Case $\alpha=\frac12$}
%
By~\cite{BFM13b}, for $\alpha=\frac12$, it is known that for $\nu \ge \pi$, with probability tending to $1$,
the random graph $G$ is connected, whereas for smaller values of $\nu$, the probability of being connected is a continuous function of $\nu$ tending to $0$ as $\nu \to 0$.

On the one hand, for any constant $\nu$, there exists a constant $C$ (with $C$ being large as $\nu$ being small) so that a.a.s.~each vertex $v\in B_{O}(R-C)$ belongs to the giant component: 
indeed, for a vertex $v\in B_{O}(i)\setminus B_{O}(i-1)$ with 
  $\frac{R}{2} < i \le R-C$, the expected number of neighbors of 
  $v$ that belong to $B_{O}(j)\setminus B_{O}(j-1)$ with say $j>\frac{R}{2}$
%  \mkc{I know its stupid, but why not $\frac{3R}{5} < j \le \frac{4R}{5}$?}
%  \dmc{I just need $i+j \ge R$ for the calculation below.}
%  \mkc{In any case, for what is being claimed up to here, one 
%  only needs $j>\frac{R}{2}$. The more restrictive bound on $j$ can
%  be required later, right?} 
  is $\Theta(e^{\frac12(R-i-j)}ne^{-\frac12(R-j)})=\Omega(1)$, where the constant 
  can be made large by making $C$ large. 
Hence, the probability that $v$ does not find 
  a neighbor in 
  $B_{O}(\frac{5R}{6})\setminus B_{O}(\frac{4R}{5})$ is $e^{-\Omega(R)}$, 
  where the constant in 
  the exponent can be made large by choosing $C$ large. 
By a similar argument, a.a.s.~every vertex in 
$B_{O}(\frac{5R}{6})\setminus B_{O}(\frac{4R}{5})$ 
  also has a neighbor in 
$B_{O}(\frac{R}{2})\setminus B_{O}(\frac{R}{4})$. 
Since all vertices within $B_{O}(\frac{R}{2})$ form a clique, all vertices 
  in $B_{O}(R-C)$ thus form a component of linear size.
Now, by choosing a sector $\Phi$ of angle $C' \log n /n$ with $C'=C'(C)$ sufficiently large, by Chernoff bounds, each such sector will a.a.s.~contain a vertex in $B_{O}(R-C)$. Hence, a.a.s.~the second component 
  has to be contained in at most two consecutive sectors, as otherwise, by Lemma~\ref{lem:FK15}, any path whose vertices are all in $B_O(R)\setminus B_O(R-C)$ spanning two sectors, as well as the component to which such path belongs, would necessarily also have to be connected to a vertex of the giant component. %\dmc{Is this enough justification?} \mkc{Do you mean ``spread out over two such adjacent sectors''? Even then, the conclusion is not immediate, right?}
Since the number of vertices in each sector of angle $C'\log n/n$ is a.a.s.~$O(\log n)$, this upper 
  bound holds also for the size of the second component.

On the other hand, for $\nu$ sufficiently small, we now show that a.a.s.~there exists a sector $\Phi$ of angle $\varepsilon \log n/n$ with $\varepsilon=\varepsilon(C)$ sufficiently small so that the following three events hold:
\begin{enumerate}[(i).-]
\item\label{it:boundary1} inside $\Phi$ there is no vertex $v$ in $B_{O}(R-C)$,
\item\label{it:boundary2} there exists a path of length $\varepsilon' \log n$ ($\varepsilon'$ sufficiently small) with all vertices being in $\varepsilon' \log n$ consecutive subsectors of $\Phi$ of angle $\varepsilon''/n$ 
  (with $\varepsilon''=\varepsilon''(C)$ small enough), 
  with all but the first and last vertex belonging to 
  $B_{O}(R-C_1+1)\setminus B_{O}(R-C_1)$ while the first and last belong 
  to $B_{O}(R-C_1)\setminus B_{O}(R-C_1-1)$ (for $C_1$ a small constant in comparison to $C$, but not too small so that any two vertices in consecutive 
  subsectors are adjacent; clearly, if  a smaller value of $C_1$ is needed below, then this can be achieved 
  by making $\varepsilon''$ smaller), 
  and except for this first and last vertex in all 
  these $\varepsilon' \log n$ subsectors there is no vertex $v$ in 
  $B_{O}(R-C_1) \setminus B_{O}(R-C)$, and %\mkc{Why do the first and last vertex of the path need to be in a different layer?}\dmc{I want to make sure that you cannot connect inside to the giant, and if connecting outside, by Lemma 8 you can do it only through first or last vertices}
\item\label{it:boundary3} no vertex of the path is connected to the giant component.
\end{enumerate} 
Note that for a fixed sector $\Phi$ condition~\eqref{it:boundary1} is satisfied with
  probability $e^{-\Theta(R)}$ with the constant in the exponent small
  for $\varepsilon$ small. 
  Condition~\eqref{it:boundary2}
  also holds with probability $e^{-\Theta(R)}$ with 
  the constant small for $\varepsilon'$ small. 
By Lemma~\ref{lem:FK15}, the last condition is satisfied if the 
  leftmost and rightmost vertex of the path do not connect to the giant 
  component, which once again happens with probability $e^{-\Theta(R)}$ 
  (again with a constant in the exponent that can be made small for $C_1$ 
  still small). 
All three conditions are either independent or positively correlated. 
Thus the expected number of sectors $\Phi$ for which all conditions hold 
  is $ne^{-\Theta(R)}/\log n=\omega(1)$ for 
  $\varepsilon, \varepsilon', \varepsilon''$ 
  sufficiently small. 
A second moment method analogous to the one in 
  Lemma~\ref{ev:G} shows that different
  sectors are "almost" independent (special care is taken of
  vertices close to the center as in Lemma~\ref{ev:H} and
  Lemma~\ref{ev:P}). 
Thus, a.a.s.~such a sector exists, so a.a.s.,~the second largest
  component is of size $\Omega(\log n)$, and 
  thus we obtain~Proposition~\ref{p:alphaHalf}.

\subsection{Case $\alpha=1$}
%
Again by~\cite{BFM15}, for $\alpha=1$, 
  for $\nu$ sufficiently large, a.a.s.~there exists a giant component,
  whereas for $\nu$ small enough, a.a.s.~the largest component is sublinear. 
Choose $\ell=\lambda R$ for some $\frac12 < \lambda < 1$ and consider 
  a vertex $v$ in $B_{O}(\ell)\setminus B_{O}(\ell-1)$ (there are 
  w.e.p.~$\Theta(ne^{-(R-\ell)})=\Theta(n^{2\lambda-1})$ such vertices). 
Since the expected number of neighbors of $v$ in $B_O(\ell)$ is 
  $\Theta(ne^{-(R-\ell)}e^{\frac12(R-2\ell)})=\Theta(1)$ 
  (where the constant can be made small enough by choosing $\nu$ 
  sufficiently small), there is a positive probability that $v$ has no 
  neighbor in $B_O(\ell)$. 

Now, for $i\in\{1,...,R-\ell\}$, 
  let $\Upsilon_{\ell+i}$ be the collection of points of 
  $B_{O}(\ell+i)\setminus B_{O}(\ell+i-1)$
  that belong to the $(2\upsilon_{\ell+i})$-sector 
  whose bisector contains the segment $Ov$ where
\[
\upsilon_{\ell+i}:=\sum_{j=0}^{i-1}\theta_R(\ell-1+j,\ell+j)
  =\Theta(e^{\frac12(R-2\ell)}).
\] 
Let $\Upsilon=\bigcup_{i=1}^{R-\ell}\Upsilon_{\ell+i}$. 
%\dmc{Changed the argument below a bit and put a bit more details. I do get dependency on $\lambda$ here}
For every vertex $v \in \Upsilon_{\ell+i}$, as before, there is a positive probability that $v$ has no 
neighbor in $B_O(\ell+i) \setminus \Upsilon$. 
A similar argument shows that there is a positive probability that $v$ has no neighbor in $B_{O}(\ell+i+d) \setminus \Upsilon$ for fixed $d > 0$. 
On the other hand, its neighbors in $B_O(\ell+i+d)$ for 
  $d$ sufficiently large must lie in $\Upsilon$: indeed, if $v$ is adjacent to a vertex $w \in B_O(\ell+i+d)$, then the angle at the origin between 
  $v$ and $w$ is $O(e^{\frac12(R-2\ell-2i-d)})$, whereas 
\[
\upsilon_{\ell+i+d}-\upsilon_{\ell+i}
  =\sum_{j=i}^{i+d-1}\theta_R(\ell-1+j,\ell+j)=\Theta(e^{\frac12(R-2\ell-2i)}),
\]
which for sufficiently large $d$ is larger than the maximum angle 
  between $v$ and $w$, and hence if 
  $v$ and $w$ are adjacent, then $w \in \Upsilon$. 

Since the number of vertices inside $\Upsilon$ is, w.e.p., 
\[
n\sum_{i=1}^{R-\ell}\mu(\Upsilon_{\ell+i})= n
  \sum_{i=1}^{R-\ell} \upsilon_{\ell+i}\mu(B_O(\ell+i)\setminus B_{O}(\ell+i-1))
  =\Theta(n^{2(1-\lambda)}),
\]
and since the events that all vertices in $\Upsilon_{\ell+i}$ have no neighbors in $B_O(\ell+i) \setminus \Upsilon$ 
  are positively correlated (also the union of all these events over all $i$), 
  with probability at least $e^{-\Theta(R)}=n^{-\gamma}$ no vertex in  $\Upsilon$ has a neighbor in $(B_{O}(R)\setminus B_{O}(\ell-1))\setminus\Upsilon$, where the constant $\gamma$ in the exponent can be made small for $\lambda$ close to $1$. 
%Arguing as in the proof of Lemma~\ref{lem:HtoG} \dmc{It should be Lemma 15, no?} one can show that 
%  with probability at least $e^{-\Theta(R)}$ no vertex in 
%  $\Upsilon$ has a neighbor in 
%  $(B_{O}(R)\setminus B_{O}(\ell-1))\setminus\Upsilon$.
%\dmc{I would comment out the following}
%Again (as in this paper) there is a probability $e^{-\Theta(R)}$
%  where the constant in the exponent can be made small for $\nu$ small enough, 
%  and for fixed $\nu$\mkc{I don't understand what ``for fixed $\nu$'' means here, isn't $\nu$ ALWAYS fixed?}, it can also be made small enough choosing 
%  $\lambda$ close to $1$\mkc{I am not getting this, in fact, I don't get a dependency on $\lambda$ for the probability! Maybe I am missunderstanding, but this parte is sort of an analogue for the $\alpha=1$ case of Lemma~\ref{ev:H}, right?}.
In this case, the original vertex $v$ is contained in a component separated 
  from the giant component (if the latter one exists) and its size is at 
  least the degree of the starting vertex, thus at least 
  $\Theta(e^{\frac12(R-\ell)})=\Theta(n^{1-\lambda})$.
%\mkc{The previous argument
%  explains the $\Omega$ part, but what about the $O(\cdot)$ part?}
%\dmc{I know. I don't have an upper bound}
  
%\dmc{added a bit}
Choosing angles sufficiently well separated and as before, taking care 
  of vertices close to the origin 
  (more precisely, on the one hand, a.a.s.~there is no vertex in 
  $B_{O}(0.49R)$, and on the other hand the angle exposed inside 
  $B_{O}(\ell) \setminus B_{O}(0.49R)$ of possible neighbors of vertices in 
  $\Upsilon$ is $\Theta(n^{1-\lambda-0.49})$; for $\lambda$ close to $1$ the 
  number of disjoint such angles is $\Theta(n^{\lambda+0.49-1})=\Omega(n^{\gamma})$ with $\gamma$ from before, and thus, 
  for $\lambda$ close to $1$, with 
  probability tending to $1$, there will be a second component of polynomial 
  size. As in the case $\frac12 < \alpha < 1$, a regrouping of $B_{O}(R)$ into groups of sectors making for a angle of $n^{-\beta}$ for $\beta > 0$ sufficiently small, the argument shows that many polynomial-size components exist (of size $\Omega(n^{\delta})$ for some $0 < \delta < \gamma$), thus establishing Proposition~\ref{p:alphaOne}. 
We do not know the exponent of the second component, though.

\section{Final remarks}
%
For $\frac12<\alpha<1$, the proof argument put forth 
  in this article does not seem 
  strong enough to be able to pinpoint the constant accompanying the
  $(\log n)^{\frac{1}{1-\alpha}}$ term in the asymptotic expression
  derived for $L_2(G)$ in Theorem~\ref{thm:main}.
We believe that developing techniques that would allow to do so
  is a worthwhile and interesting endeavor.

%  LocalWords:  Chernoff mk subsectors sublinear


==> secIntro.tex <==
\section{Introduction}\label{sec:intro}
%
The model of random hyperbolic graphs introduced by Krioukov et al.~\cite{KPKVB10} has attracted quite a bit of interest due to its key properties also observed in large real-world networks. One convincing demonstration of this fact was given by Bogu\~n\'{a} et al.~in~\cite{BPK10}
  where a compelling (heuristic)
  maximum likelihood fit of autonomous systems of the internet graph in hyperbolic 
  space was computed. A second powerful reason for why the model  
  initially caught attention is due to the 
  experimental results reported by Krioukov et al.~\cite[\S~X]{KPKVB10} confirming that the model exhibits
  the algorithmic small-world phenomenon established
  by the groundbreaking letter forwarding experiment of Milgram from 
  the 60's~\cite{Mil67}.

\medskip
Another important aspect of the random graph model introduced 
  in~\cite{KPKVB10} is its mathematically elegant specification and the 
  fact that it is amenable to mathematical analysis.
This partly explains why the model has been studied not only empirically 
  by the networking community but also analytically by theoreticians.
For the latter, it is natural to first consider those issues that
  played a crucial role in the development of the theory of 
  other random graph models.
Among these, the Erd\H{o}s-R\'{e}nyi random graph model is undisputedly 
  the most relevant. 
One of the most, if not the most, studied aspect of the Erd\H{o}s-R\'{e}nyi model
  is the evolution (as a function of the graph density) 
  of the size and number of its connected components~\cite{ER60}, specially the 
  size of the largest one, but also the size of the second largest.
These studies have played a crucial role in the development of 
  mathematical techniques and significantly contributed to the understanding
  of the Erd\H{o}s-R\'{e}nyi random graph model.
For the random hyperbolic graph model, the study of the largest 
  component's size was started by Bode, Fountoulakis and M\"{u}ller~\cite{BFM13}
  and recently refined by Fountoulakis and M\"{u}ller~\cite{FMLaw}.
A logarithmic lower bound and polylogarithmic upper bound 
  for the size of the second largest component of random
  hyperbolic graphs (when $\frac12<\alpha<1$) were first established 
  in~\cite{KM17}.
In this note we improve on these bounds and determine the 
  precise order of the size 
  of the second largest component of random hyperbolic graphs.


\bigskip\noindent
\textbf{Model specification:}
In the original model of Krioukov et al.~\cite{KPKVB10} an $n$-vertex size graph $G$ was obtained by first randomly choosing $n$ points in $B_{O}(R)$ (the disk of radius $R=R(n)$ centered at the origin $O$ of the hyperbolic plane).
From a probabilistic point of view it is arguably more natural to consider the Poissonized version of this model. Formally, the Poissonized model 
%\mkc{Does [GPP12] actually talk about Poissonization? Needs checking.}\dmc{No. GPP12 does not Poissonize it. So I changed it a bit.} 
is the following (see also~\cite{GPP12} for the same description in the uniform model): for each $n \in \NN$, we consider a Poisson point process on the hyperbolic disk of radius $R :=2 \log (n/\nu)$ for some positive constant $\nu \in \RR^+$ ($\log$ denotes here and throughout the paper the natural logarithm) and denote its point set by $V$ (the choice of $V$ is due to the fact that we will identify points of the Poisson process with vertices of the graph). The intensity function at polar coordinates $(r,\theta)$ for 
  $0\leq r< R$ and $0 \leq \theta < 2\pi$ is equal to
\[
g(r,\theta) := \nu e^{\frac{R}{2}}f(r,\theta),
\]
where $f(r,\theta)$ is the joint density function with $\theta$ chosen uniformly at random in the interval $[0,2\pi)$ and independently of $r$ chosen according to the density function
\begin{align*}
f(r) & := \begin{cases}\displaystyle
   \frac{\alpha\sinh(\alpha r)}{\cosh(\alpha R)-1}, &\text{if $0\leq r< R$}, \\
   0, & \text{otherwise}.
  \end{cases}
\end{align*}
Identify then the points of the Poisson process with vertices (that is, for each vertex $v \in V$ we identify it with its position in polar coordinates $(r_v,\theta_v)$) and make the following graph $G=(V,E)$: for $u, u'\in V$, $u \neq u'$, there is an edge with endpoints 
  $u$ and $u'$ provided the distance (in the hyperbolic plane) between
  $u$ and $u'$ is at most $R$, i.e.,  
  the hyperbolic distance
  between $u$ and $u'$, denoted by 
  $\dist:=\dist(u,u')$,
  is such that  $\dist\leq R$ where $\dist$ is obtained by solving 
\begin{equation}\label{eqn:coshLaw}
\cosh \dist := \cosh r_u\cosh r_{u'}-
  \sinh r_u\sinh r_{u'}\cos( \theta_u{-}\theta_{u'}).
\end{equation}


For a given $n \in \NN$, we denote this model by 
  $\poimod_{\alpha,\nu}(n)$.
Note in particular that 
\[
\iint g(r,\theta) d\theta dr 
  = \nu e^{\frac{R}{2}}=n,
\]
and thus  $\EE|{V}|=n.$ 
  The main advantage of defining $V$ as a Poisson point process is
  motivated by the following two properties: the number of points of
  $V$ that lie in any region $A \subseteq B_O(R)$ follows a Poisson
  distribution with mean given by $\int_A g(r,\theta) drd\theta=n
  \mu(A)$, and the numbers of points of $V$ in disjoint
  regions of the hyperbolic plane are independently distributed.
  %Moreover, by conditioning $\layer$ upon the event $|{\layer}|=n$, we recover the original distribution. 
  
%  Therefore, since
%  $\Pr(|{\layer}|=n-k)=\Theta(1/\sqrt n)$ for any $k=O(1)$, any event
%  holding in $\layer$ with probability at least $1-o(f_n)$ must hold in
%  the original setup with probability at least $1-o(f_n \sqrt n)$, and
%  in particular, any event holding with probability at least
%  $1-o(1/\sqrt{n})$ holds a.a.s.~in the
%  original model. Also, an event holding w.e.p.~in 
%  $\poimod_{\alpha,C}(n)$ also holds w.e.p.~in $\unifmod_{\alpha,C}(n)$.  
%Henceforth, unless stated otherwise, our results will be presented in the Poissonized model only; the corresponding results for the uniform model follow by the above considerations.

%The impressive quality of the embedding obtained is an
%  indication that hyperbolic geometry underlies 
%  important real networks.
%This partly explains the considerable interest the model has
%  attracted since its introduction.

%Formally, the random hyperbolic graph model $\unifmod_{\alpha,C}(n)$ is defined
%  in~\cite{GPP12} as described next: for $\alpha> \frac12$, $C\in\RR$, $n\in\NN$, set $R=2\log n+C$ ($\log$ denotes here and throughout the paper the natural logarithm), and 
%  build $G=(V,E)$ with vertex set $V$ a subset of $n$ points
%  of the hyperbolic plane $\HH^2$ chosen as follows:
%\begin{itemize}
%\item For each $v\in V$, polar coordinates $(r_{v},\theta_{v})$ are 
%  generated identically and independently distributed with joint
%  density function $f(r,\theta)$, with $\theta_{v}$ chosen uniformly 
%  at random in the interval $[0,2\pi)$ and $r_{v}$ with density:
%
%
%\item \end{itemize}
The restriction $\alpha>\frac12$ and the role of $R$, informally speaking,
  guarantee that the resulting graph has bounded average degree (depending
  on $\alpha$ and $\nu$ only): if $\alpha<\frac12$, then the degree sequence is so 
  heavy tailed that this is impossible (the graph is with high probability connected in this case, as shown in~\cite{BFM13b}), and if $\alpha>1$, then
  as the number of vertices grows,
  the largest component of a random hyperbolic graph has sublinear 
  order~\cite[Theorem~1.4]{BFM15}.
In fact, although some of our results hold for a wider range of $\alpha$, 
  we will always assume $\frac12<\alpha<1$; only in the concluding remarks we discuss the cases $\alpha=\frac12$ and $\alpha=1$.
  %, since as already discussed, this is the most interesting regime.
  
%\medskip
%A common way 
%  of visualizing the hyperbolic plane $\HH^2$ is via its
%  native representation where the choice for 
%  ground space is $\RR^2$.
%Here, a point of $\RR^2$ with polar coordinates $(r,\theta)$ has 
%  hyperbolic distance to the origin $O$ equal to its Euclidean distance~$r$.
%In the native representation, an instance of $\unifmod_{\alpha,C}(n)$
%  can be drawn by mapping a vertex $v$ to the point in $\RR^2$ with polar
%  coordinate $(r_v,\theta_v)$ and drawing edges as straight lines.
%Clearly, the graph drawing will lie within $B_{O}(R)$ 
%  (see Figure~\ref{fig:hyperGraph}).
%
%\begin{figure}[ht]
%\begin{center}
%\scalebox{0.75}{\includegraphics{giantComp-a55-C2-25-n740-m633.png}}
%\end{center}
%\caption{Native representation of the largest connected component 
%  (with $621$ vertices) of an instance of a graph with $\alpha=0.55$, $C=2.25$ and $n=740$.
%The solid (respectively, segmented) circle is the boundary of 
%  $B_{O}(R)$ (respectively, $B_{O}(\frac{R}{2})$).}\label{fig:hyperGraph}
%\end{figure}

%\medskip
%The adjacency, Laplacian, and normalized Laplacian
%  are three well-known matrices associated to a graph, 
%  all of whose spectrum encode important information 
%  related to fundamental graph parameters.
%For non-regular graphs, such as a random hyperbolic graph $G=(V,E)$
%  obtained from $\unifmod_{\alpha,C}(n)$, 
%  arguably the most relevant associated matrix is the 
%  normalized Laplacian $\calL_G$. Note
%  that $\calL_G$ is positive semidefinite and has 
%  smallest eigenvalue $0$.
%Certainly, the most interesting parameter of 
%  $\calL_G$ is its eigenvalue gap $\lambda_1(G)$.
%Since for $\frac12<\alpha<1$,
%  a typical occurrence of $G$ has $\Theta(|V|)$ isolated vertices,
%  the eigenvalue $0$ of $G$ has high multiplicity
%  and thus $\lambda_1(G)=0$.
It is known that for $\frac12 < \alpha < 1$, with high probability the 
  graph $G$ has a linear size 
  component~\cite[Theorem~1.4]{BFM15}  
  and all other components are of
  polylogarithmic order~\cite[Corollary 13]{km15}, 
  which justifies referring to the
  linear size component as \emph{the giant component}.
Implicit in the proof of~\cite[Theorem 1.4]{BFM15} is that the giant component of a
  random hyperbolic graph $G$ is the one
  that contains all vertices whose radial coordinates are at most $\frac{R}{2}$. More
  precise results including a law of large numbers for the largest
  component in these networks were established recently
  in~\cite{FMLaw}. 

\bigskip\noindent
\textbf{Main result and proof overview:}
In this note we determine the exact order of 
  the size of the second largest component, which we denote by $L_2(G)$. 

\bigskip
We say that an event holds \emph{asymptotically almost surely (a.a.s.)}, if it holds with probability tending to $1$ as $n \to \infty.$ 
The main result of this note is the following:
\begin{theorem}\label{thm:main}
Let $\frac12 < \alpha < 1$. Let $G=(V,E)$ be chosen according to $\poimod_{\alpha,\nu}(n)$. A.a.s.,
\[
L_2(G)=\Theta(\log^{\frac{1}{1-\alpha}} n).
\]
Moreover, for some sufficiently small constant $b>0$, there are 
  $\Omega(n^{b})$ components in $G$, each one of size 
  $\Theta(\log^{\frac{1}{1-\alpha}} n)$.
\end{theorem}
To establish the lower bound, we partition the disk into sectors, so that close to the central axis of each sector, one can find a chain (a path) of vertices at a certain distance from the boundary so that the expected number of vertices with larger radius and in the same sector is of the desired order. While it is relatively easy to show that a constant fraction of these vertices indeed connects to the chain, it is more work to show that none of these vertices in fact is connected to the giant component. Technically, this is tedious since vertices at all radii might potentially be connected to the giant component; vertices with smaller radii might be more dangerous to have neighbors with smaller radii, whilst vertices with bigger radii (close to the border) might be more dangerous to have neighbors with larger radii.

\medskip

An original aspect of our lower bound 
  analysis consists in identifying ``walls'', that is, 
  regions $\calW$, inside $B_{O}(R)$ and close to 
  its boundary (specifically, a 
  collection of connected points at 
  distance at least $\ell:=R-O(\log R)$ 
  from the origin) which satisfy the following conflicting
  properties: 
  (i) they do not contain vertices, and
  (ii) for a sector  
  $\Phi$ of $B_{O}(R)$ strictly containing $\calW$,
  the region $\Phi\setminus B_{O}(\ell)$ 
  is partitioned into connected regions
  $\calW',\calW,\calW''$
  in such a way that the hyperbolic distance between a point in 
  $\calW'$ and a point in $\calW''$ is greater than $R$. 
The abundance of walls coupled
  with the fact that the subgraph of $G$ induced
  by the vertices in $B_{O}(R)\setminus B_{O}(\ell)$ contains,
  many connected components (which we refer to as \emph{pre-components})
  reduces the problem of bounding $L_2(G)$ from below to one of showing that there are regions of $B_O(\ell)$ which are 
  unlikely to contain vertices of $G$ (these latter regions are the
  ones where neighbors of pre-components can potentially lie).

Interestingly, the mentioned abundance of walls also explains 
  the ``forest-like'' structure close to the boundary of 
  $B_{O}(R)$ that random hyperbolic graphs exhibit 
  (see Figure~\ref{fig:forest}). 
\begin{figure}[ht]
\def\vertRad{1pt}
\subfloat[][]{\centering\input{fig1.inc}}
\hfill
\subfloat[][]{\centering\input{fig2.inc}}
\caption{(Left) An instance $G$ of Krioukov et.~al.'s 
  random hyperbolic graph model with parameters $n=1000$, $\alpha=0.7$,
  and $\nu=1.1$.
  (Right) The subgraph of $G$ induced by the vertices inside the dashed region shown on the left side, where angular coordinates have been scaled by factor of $6$ in order to better elicit the forest-like structure of the induced graph.}\label{fig:forest}
\end{figure}

\medskip 
  The upper bound of Theorem~\ref{thm:main}, comparably easier, makes use of the fact that all vertices that are not too close to the boundary of $B_O(R)$ belong to the giant component. We can thus find in every sector of not too big angle a vertex belonging to the giant component, and by simple known geometric observations any other component must be squeezed between two such sectors. Since the number of vertices in such a sector is concentrated, we get an upper bound on the size of the second component.


\medskip
To conclude our study of the size of the second largest component of 
  random hyperbolic graphs we consider the relevant remaining cases where 
  $\alpha=\frac12$ or $\alpha=1$.
In the former case, we show that a.a.s.~every vertex of the 
  second largest component must be within
  $C=\Theta(1)$ of the boundary of $B_{O}(R)$.
Moreover, by some geometric considerations, such component must 
  be contained in a sector $\Phi$ of $B_{O}(R)$ 
  for which $\Phi\cap B_{O}(R-C)$ does
  not contain vertices of $G$.
An analysis of the likely maximum angle such a sector $\Phi$ can have 
  and of the number of vertices that can be found in 
  $\Phi \setminus B_{O}(R-C)$ yields the following:
\begin{proposition}\label{p:alphaHalf}
For $\alpha=\frac12$, a.a.s.,~$L_2(G)=\Theta(\log n)$.
\end{proposition}
For the $\alpha=1$ case, we show that a.a.s.~there is $\frac12<\lambda<1$ and a vertex of degree $\Theta(n^{1-\lambda})$ that belongs to a component separated from the giant, so we obtain the following:
\begin{proposition}\label{p:alphaOne}
For $\alpha=1$ there exists $\gamma$, $0<\gamma<1$ such that 
  a.a.s.,~$L_2(G)=\Omega(n^{\gamma})$. 
Moreover, for some $0 < \delta < \gamma$ and for some sufficiently small constant $b>0$, a.a.s.~there are $\Omega(n^b)$ components in $G$, each one of size $\Omega(n^{\delta})$.
\end{proposition}

\bigskip\noindent
\textbf{Related work:}
Although the random hyperbolic graph model was relatively
  recently introduced~\cite{KPKVB10}, several of its key properties have already been established. As already mentioned, in~\cite{GPP12}, the degree distribution, the expected value of the maximum degree and global 
  clustering coefficient were determined, and in~\cite{BFM15}, the existence of a giant component as a function of $\alpha$.
  
  The threshold in terms of $\alpha$ for the connectivity of random
  hyperbolic graphs was given in~\cite{BFM13b}. 
Concerning diameter and graph distances,
  except for the aforementioned papers of~\cite{km15} and~\cite{fk15},
  the average distance of two points belonging to the giant component
  was investigated in~\cite{ABF}. 
Results on the global clustering coefficient of the so called
  binomial model of random hyperbolic graphs were obtained
  in~\cite{CF13}, and on the evolution of graphs on more general
  spaces with negative curvature in~\cite{F12}. 
Finally, the spectral gap of the Laplacian of this model was studied 
  in~\cite{KM17}

The model of random hyperbolic graphs for $\frac12 < \alpha < 1$ is very similar to two different models
studied in the literature: the model of inhomogeneous long-range
percolation in $\ZZ^d$ as defined in~\cite{Remco}, and the
model of geometric inhomogeneous random graphs, as introduced
in~\cite{BKL2}. In both cases, each vertex is given a weight, and
conditionally on the weights, the edges are independent (the presence
of edges depending on one or more parameters). In~\cite{Remco} the
degree distribution, the existence of an infinite component and the
graph distance between remote pairs of vertices in the model of
inhomogeneous long-range percolation are analyzed. On the other hand,
results on typical distances, diameter, clustering coefficient,
separators, and existence of a 
  giant component in the model of geometric
inhomogeneous graphs were given in~\cite{BKL1,BKL2}, bootstrap
percolation in the same model was studied in~\cite{KL} and 
  greedy routing in~\cite{BKLMM17}. Both models
are very similar to each other, and similar results were obtained in
both cases; since the latter model assumes vertices in a toroidal
space, it generalizes random hyperbolic graphs.  


\bigskip\noindent\textbf{Notation:}
All asymptotic notation in this paper is respect to $n$. Expressions given in terms of other variables such as $O({R})$ are still asymptotics with respect to $n$, since these variables still depend on $n$.
We say that an event holds \emph{with extremely high probability
    (w.e.p.)}, if for every $c > 0$, there exists an $n_0:=n_{0}(c)$
  such that for every $n\geq n_0$ the event holds with
  probability at least $1-O(n^{-c})$. 
Note that the union of polynomially (in $n$) many events (where the degree 
  of the polynomial is not allowed to depend on $c$) that hold w.e.p.~is 
  also an event that holds w.e.p. In what follows, any union bound 
  is over at most $O(n^2)$ many events. 
%\mk{In order to reduce the number of parameters we work with, throughout 
%  this article, when aiming to show a claim holds w.e.p., 
%  we just show that for an appropriate choice of constants, 
%  the event holds with probability at least $1-n^{-100}$, with
%  the implicit understanding that we can replace $100$ by any other 
%  power simply by changing the choice of relevant constants.}t

%  LocalWords:  Krioukov et al Fountoulakis Poissonized subgraph mk
%  LocalWords:  polylogarithmic Laplacian inhomogeneous toroidal


==> secPrelim.tex <==
\section{Preliminaries}\label{sec:prelim}
%
In this section we collect some of the known properties concerning 
  random hyperbolic graphs. 
  
\medskip
By the hyperbolic law of cosines~\eqref{eqn:coshLaw}, 
  the hyperbolic triangle formed by the geodesics 
  between points $p'$, $p''$, and  $p$, with opposing side segments of length 
  $\distp$, $\distpp$, and $\dist$ respectively,
  is such that the angle formed at $p$ is:
\begin{equation*}\label{eqn:angle}
\theta_{\dist}(\distp,\distpp) = 
\arccos\Big(\frac{\cosh \distp\cosh \distpp-\cosh \dist}{\sinh \distp\sinh \distpp}\Big).  
\end{equation*}
Clearly, $\theta_{\dist}(\distp,\distpp) = \theta_{\dist}(\distpp,\distp)$. 
\begin{remark}\label{rem:monotonTheta}
Recall that $\cosh(\cdot)$ is at least $1$ and strictly increasing
  in $\RR^+$.
Moreover, $\cosh^2 x-\sinh^2 x=1$.
Hence, if $0<x, y\leq R$, then
\[
\frac{\partial}{\partial x}\Big(\frac{\cosh x\cosh y - \cosh R}{\sinh x\sinh y}\Big)
  = \frac{-\cosh y+ \cosh R\cosh x}{\sinh^2 x\sinh y}
  > \frac{\cosh R-\cosh y}{\sinh^2 x\sinh y}
  \geq 0.
\]
Since $\arccos(\cdot)$ is strictly decreasing, it follows that 
  $\theta_{R}(\cdot,y)$ is strictly decreasing for fixed $0<y\leq R$.
By symmetry, a similar claim holds for 
  $\theta_{R}(x,\cdot)$.
\end{remark}


Next, we state a very handy approximation for $\theta_{R}(\cdot,\cdot)$.
\begin{lemma}[{\cite[Lemma 3.1]{GPP12}}]\label{lem:aproxAngle}
If $0\leq\min\{\distp,\distpp\}\leq R \leq \distp+\distpp$, then
\[
\theta_{R}(\distp,\distpp) = 2e^{\frac{1}{2}(R-\distp-\distpp)}\big(1+\Theta(e^{R-\distp-\distpp})\big).
\]
\end{lemma}
\begin{remark}\label{rem:aproxAngle}
We will use the previous lemma also in this form: let
  $p'$ and $p''$ be two points at distance $R$ from each other
  such that $r_{p'},r_{p''} > \frac{R}{2}$ and $\min\{r_{p'},r_{p''}\}  \leq R$.
Then, taking $\distp=r_{p'}$
  and $\distpp=r_{p''}$ in Lemma~\ref{lem:aproxAngle}, we get
\[
\theta_{R}(r_{p'},r_{p''}) 
  := 2e^{\frac{1}{2}(R - r_{p'} - r_{p''})}\big(1+\Theta(e^{R-r_{p'}-r_{p''}})\big).
\]
%Note also that $\theta_{\dist}(r_{p'},r_{p''})$, for fixed $r_{p'},r_{p''} > \frac{R}{2}$, 
  %is increasing as a function of $\dist$ (for $\dist$ satisfying the constraints). 
%Below, when aiming for an upper bound, we always use $\dist=R$.
\end{remark}

\medskip
Throughout, we will need estimates for measures of 
  regions of the hyperbolic plane, and more specifically, for regions obtained by performing some set algebra
  involving a few balls.
For a point $p$ of the hyperbolic plane $\HH^2$, 
  the ball of radius $\rho$ centered at $p$ will be denoted by
  $B_{p}(\rho)$, i.e., 
  $B_{p}(\rho) := \{q\in\HH^2 : \dist(p,q)\leq\rho\}$.

Also, we denote by $\mu(S)$ the measure of a set 
  $S \subseteq \HH^2$, i.e.,
  $\displaystyle\mu(S) := \int_{S}f(r,\theta)drd\theta$.

Next, we collect a few results for such measures.
\begin{lemma}[{\cite[Lemma~3.2]{GPP12}}]\label{lem:muBall} 
If $0\leq \rho< R$, then
  $\mu(B_{O}(\rho)) = e^{-\alpha(R-\rho)}(1+o(1))$.
%Moreover, if $p\in B_{O}(R)$, then for 
%  $C_{\alpha}:=2\alpha/(\pi(\alpha-\frac{1}{2}))$,
%\begin{equation}\label{eq:muBall2}
%\mu(B_{p}(R)\cap B_{O}(R)) = C_{\alpha}e^{-\frac{r_p}{2}}\big(1+O(e^{-(\alpha-\frac{1}{2})r_p}+e^{-r_p})\big).
%\end{equation}
\end{lemma}
A direct consequence of Lemma~\ref{lem:muBall} is
\begin{cor}\label{cor:medidalb} 
If $0 \leq \rho'_O < \rho_O < R$, then
\[
\mu(B_{O}(\rho_{O})\setminus B_{O}(\rho'_{O}))
  = e^{-\alpha(R-\rho_{O})}(1-e^{-\alpha(\rho_{O}-\rho'_{O})}+o(1)).
\]
\end{cor}
By a simple application of Chernoff bounds, we have the following lemma:%
\begin{lemma}[{\cite[Lemma~12]{KM17}}]\label{lem:Poisson}
Let $V$ be the vertex set of a graph chosen according to $\poimod_{\alpha,\nu}(n)$. 
For every $c>0$, there is a sufficiently large
  constant $c'=c'(c)$ 
  such that if $S\subseteq B_{O}(R)$ with $\mu(S)\ge c'\log n/n$,
  then with probability at least $1-n^{-c}$,
  $|S\cap V|=\Theta (n \mu(S)).$ If moreover $S \subseteq B_{O}(R)$ is such that $\mu(S) = \omega(\log n/n)$, then w.e.p.~$|S\cap V|=\Theta (n \mu(S)).$ 
\end{lemma}
We need one more lemma.

\begin{lemma}[{\cite[Lemma~9]{fk15}}]\label{lem:FK15}
Let $p,p',p''\in B_{O}(R)$ be such that $\theta_{p} \le \theta_{p'} \le \theta_{p''}$ and let $\dist(p,p'')\leq R$. 
Then the following holds: 
  if $r_{p'} \le \min\{r_{p},r_{p''}\}$, then 
  $\dist(p,p'),\dist(p',p'')\leq R$.
\end{lemma}



\section{Intermediate regime of $\alpha$}\label{sec:proofs}
%
In this section we prove the main result of this article which concerns
  the regime where $\alpha$ takes values strictly between $\frac12$ and $1$. 
Since our results are asymptotic, we may and will ignore floors in the 
  following calculations, and assume that certain expressions such as 
  $R-\frac{\log R}{1-\alpha}$, $R-\frac{\log R}{1-\alpha}-\frac{L}{1-\alpha}$ 
  for some constant $L$ or the like are integers, if needed.
  When working with a Poisson point process $V$, for a positive 
  integer $\ell$, we refer to the vertices of $G$ that belong to 
  $B_{O}(\ell)\setminus B_{O}(\ell-1)$ as the $\ell$-th \emph{band} or \emph{layer} and 
  denote it by $\layer_{\ell}:=\layer_{\ell}(G)$, i.e.,  
  $\layer_{\ell}=V \cap B_{O}(\ell)\setminus B_{O}(\ell-1)$.
%\mkc{It seems to me it would be better notation to use $V_{\ell}$ instead 
%  of $\layer_{\ell}$.} \dmc{Ok. Change it please}
Throughout this section we always assume that $\frac12<\alpha<1$.

\subsection{Upper bound}
%
We start with an observation that simplifies arguing about the giant component of random hyperbolic graphs. A similar but slightly weaker result was already proven in~\cite{KM17}.
\begin{lemma}\label{lem:HtoG}
Let $\ell:= R-\frac{\log R}{1-\alpha}-\frac{L}{1-\alpha}$ and $G=(V,E)$ 
  be chosen according to $\poimod_{\alpha,\nu}(n)$. 
For every $c>0$, there is a 
  sufficiently large constant $L:=L(c)>0$ such that 
  with probability at least $1-O(n^{-c})$, all vertices in 
  $V \cap B_O(\ell)$ belong to the giant component.
  % and hence, for each $\ell \le R-\frac{\log R}{1-\alpha}-\frac{L}{1-\alpha}$, w.h.p.~$\layer_{\ell}(G)=\layer_{\ell}(H).$
\end{lemma}
\begin{proof}
First observe that by~\cite{BFM15}, w.e.p.~every vertex $v \in \layer_{i}$ with $i \le\frac{R}{2}$ belongs to the giant component. 
Hence, it suffices to show that for a sufficiently large $L$ and 
  every vertex $v\in\layer_{i}$ with $\frac{R}{2} \le i\le \ell$ with 
  probability at least $1-O(n^{-c})$, there exists a path connecting 
  $v$ to a vertex in $V \cap B_O(\frac{R}{2})$. 
Taking a union bound, and iterating the argument
  with $i-1$ instead of $i$ until $i=\frac{R}{2}$, 
  it is enough to show that 
  for a fixed vertex $v\in\layer_i$ with $i$ as before,
  with probability at least $1-O(n^{-(c+1)})$, vertex $v$ has a neighbor 
  in $\layer_{i-1}$. Indeed, by Remark~\ref{rem:aproxAngle}, $v$ is connected to vertex $u \in \layer_{i-1}$ if the angle at the origin between $u$ and $v$ is 
  $O(\theta_R(i,i))$. 
By Corollary~\ref{cor:medidalb}, we have
\[
\mu(B_{v}(R)\cap B_{O}(i-1)\setminus B_O(i-2)) =\Theta(e^{-\alpha(R-i)}e^{\frac12(R-2i)})=\Theta(e^{(1-\alpha)(R-i)}/n).
\]
Since $\alpha < 1$, this expression is clearly decreasing in $i$, and plugging in our upper bound on~$i$, we obtain
\[
\mu(B_{v}(R)\cap B_{O}(i-1)\setminus B_O(i-2)) =\Omega(e^{(R-\ell)(1-\alpha}/n)=\Omega(\log n/n),
\]
where the constant hidden in the asymptotic expression can be made arbitrarily large by choosing $L$  large enough so that applying Lemma~\ref{lem:Poisson} guarantees that with probability at least $1-O(n^{-(c+1)})$, vertex $v$ has 
  $\Omega(\log n)$ neighbors in $\layer_{i-1}$. 
By definition, $v$ is connected by an edge to any such vertex, and hence in 
  particular with probability at least $1-O(n^{-(c+1)})$, vertex $v$ 
  has a neighbor in $\layer_{i-1}$. 
\end{proof}

Define next a $\phi$-sector $\Phi$ to be a sector of $B_O(R)$, that contains all points in $B_O(R)$ making an angle of at most $\phi$ at the origin with an arbitrary but fixed reference point. 

We deduce from the previous lemma that in any not too small angle there will be at least one vertex belonging to the giant component:
\begin{lemma}\label{lem:maxAngle}
For every $c>0$, there are sufficiently large positive constants 
  $L:=L(c)$ and $L':=L'(c)$, such that for 
  $\ell:= R-\frac{\log R}{1-\alpha}-\frac{L}{1-\alpha}$
  and $\phi :=\frac{L'}{n}(\log n)^{1/(1-\alpha)}$,
  with probability at least $1-O(n^{-c})$,
  every $2\phi$-sector $\Phi$ contains at least one vertex 
  $v \in \layer_{\ell}$.
\end{lemma}
\begin{proof}
By Lemma~\ref{lem:HtoG}, for $L$ sufficiently large, with probability at 
  least $1-O(n^{-c})$, 
  all vertices in $B_O(\ell)$ belong to the giant component. 
Partition $B_O(R)$ into $\phi$-sectors $\Phi_1, \ldots, \Phi_{2\pi/\phi}$. 
By Corollary~\ref{cor:medidalb}, we get
\[
\mu(\Phi_i\cap B_O(\ell)\setminus B_{O}(\ell-1))
  = \Theta(\phi e^{-\alpha(R-\ell)})=\Theta(\log n/n).
\]
For $L'$ sufficiently large, the constant hidden in the asymptotic notation 
  can be made as large as required by Lemma~\ref{lem:Poisson} to get that, 
  with probability at least $1-O(n^{-(c+1)})$, the number of vertices in 
  $\layer_{\ell}\cap\Phi_{i}$ is $\Theta(\log n)$. 
By taking a union bound over all  $\phi$-sectors $\Phi_i$ 
  (there are $2\pi/\phi=O(n)$ of them), this holds with probability at 
  least $1-O(n^{-c})$ in all of them simultaneously. 
The statement then follows since every $2\phi$-sector $\Phi$ has to contain 
  entirely a $\phi$-sector $\Phi_i$, and by a union bound over all events.
\end{proof}
We are now ready for the upper bound on the second largest component.
\begin{proposition}\label{p:UpperBound}
Let $G=(V,E)$ be chosen according to $\poimod_{\alpha,\nu}(n)$. W.e.p., 
\[
L_2(G) = O(\log^{\frac{1}{1-\alpha}} n).
\]
\end{proposition}
\begin{proof}
Let $c>0$.
Let $\ell:=\ell(L)$, $L:=L(c+1)$, $\phi:=\phi(L')$, and $L':=L'(c+1)$
  be as in the statement of Lemma~\ref{lem:maxAngle}.
By a union bound and appropriate choices of $L$ and $L'$, 
Lemma~\ref{lem:HtoG} and Lemma~\ref{lem:maxAngle} imply that, 
  with probability at least $1-O(n^{-(c+1)})$, all vertices in $B_{O}(\ell)$
  belong to the giant component and 
  every $2\phi$-sector contains at least one vertex $v\in B_{O}(\ell)$.
Henceforth, condition on the latter event. Then, every vertex $x$ outside 
  the giant component belongs to $B_{O}(R)\setminus B_{O}(\ell)$. Now, consider a component $C$ distinct from the giant component and let $u,u'$ be vertices in $C$ such that
  $|\theta_{u'}-\theta_{u}|=\max_{x,x'} |\theta_x-\theta_{x'}|$, where the 
  maximum is taken over all pairs of vertices $x,x'$ belonging to $C$.
If we had $|\theta_{u'}-\theta_{u}| \ge 2\phi$ 
  then by our conditioning there would be a vertex $v\in B_{O}(\ell)$
  (thus in the giant component) such that 
  $\theta_{u} \le \theta_v \le \theta_{u'}$.
Since there exists a path in $C$ between $u$ and $u'$ containing only vertices 
  $u_j$ with $r_{u_j} > \ell$, in such a path there must be a pair of 
  vertices, say $u_i, u_j$, with 
  $r_v \le r_{u_i}, r_{u_{j}}$, $u_iu_{j} \in E$, and 
  $\theta_{u_i} \le \theta_v \le \theta_{u_{j}}$.
By Lemma~\ref{lem:FK15}, then however, also $u_iv \in E$ and $u_{j}v \in E$, 
  and hence $u$ and $u'$ are connected to the giant component. 
Therefore, by our conditioning we may assume that $|\theta_{u'}-\theta_{u}| < 2\phi$. 
Note that conditioning on Lemma~\ref{lem:HtoG} and Lemma~\ref{lem:maxAngle} 
  does not change the distribution of vertices in $B_{O}(R)\setminus B_{O}(\ell)$. 
Hence, since $\phi=\omega(\log n/n)$, by Lemma~\ref{lem:Poisson}, 
  w.e.p.~we get $|C|=O(\phi n)=O((\log n)^{\frac{1}{1-\alpha}})$. 
By a union bound over all events, 
  with probability at least $1-O(n^{-c})$, it holds 
  that $L_2(G) = O((\log n)^{\frac{1}{1-\alpha}})$ and the statement follows.
\end{proof}

\subsection{Lower bound}\label{subs:Lower}
%
We next turn to prove a lower bound matching the bound of Proposition~\ref{p:UpperBound}. Let $M=M(\alpha, \nu)$ throughout this subsection be a sufficiently large constant. Partition $B_O(R)$ into $\psi$-sectors with $\psi:=(\nu/n)^{1-\beta}$ for a sufficiently small constant $\beta=\beta(\alpha, M, \nu)$ (first, $M$ has to be chosen sufficiently large as a function of the model parameters $\alpha$ and $\nu$, independent of $\beta$, and then, $\beta$ has to be chosen small enough). 
Fix throughout this subsection 
  $\ell:=R-\frac{\log R}{1-\alpha}+\frac{M}{1-\alpha}$ 
  (recall that we suppose that $\ell$ is an integer). 
Let $\phi := 9\theta_{R}(\ell,\ell)$.
By Lemma~\ref{lem:aproxAngle} and since $R=2\log\frac{n}{\nu}$,
\begin{equation}\label{eqn:phi}
\theta_{R}(\ell,\ell) = (2+o(1))\frac{\nu}{n}e^{R-\ell}
  = (2+o(1))\frac{\nu}{n}R^{\frac{1}{1-\alpha}}e^{-\frac{M}{1-\alpha}}.
\end{equation}
%Note that $\varepsilon \to 0$ as $M=M(\alpha,\nu) \to \infty$. 
For each $\psi$-sector $\Psi$, consider the region 
  $\Upsilon_{\ell}:=\Upsilon_{\ell}(\Psi)$ consisting of those points  
  of $B_{O}(\ell)\setminus B_{O}(\ell-1)$ that belong to the 
  $\phi$-sector having the same bisector as $\Psi$.
Next, we establish a lower bound on the probability that  
  $V\cap\Upsilon_{\ell}$ induces a connected component of $G$. 
Actually, we establish a stronger fact.
In the ensuing discussion, unless we say otherwise, the $\psi$-sector
  $\Psi$ is assumed to be given and all regions as well as subgraphs
  mentioned depend on $\Psi$.
\begin{lemma}\label{ev:B}
Let $\Upsilon'_{1},\ldots,\Upsilon'_{18}$ be a partition
  of $\Upsilon_{\ell}$ into $18$ parts, 
  each $\Upsilon'_{i}$
  obtained as the intersection of $\Upsilon_{\ell}$ and a 
  $\frac{\phi}{18}$-sector.
The following hold:
\begin{enumerate}[(i).-]
\item\label{it:B1}
Let $\calB$ be the event that $\layer\cap\Upsilon'_{i}$
  is non-empty for every $i=1,...,18$.
Then, $\calB$ occurs a.a.s.
%Moreover, all area exposed in $\calB$ is inside $\Upsilon_{\ell}$.

\item\label{it:B2}
For sufficiently large $n$, conditioned on $\calB$, all vertices in 
  $\layer\cap\Upsilon_{\ell}$ belong to the same connected component.
\end{enumerate}
\end{lemma}
\begin{proof}
To prove~\eqref{it:B1}, observe that by our choice of $\phi$,
  Corollary~\ref{cor:medidalb}, and~\eqref{eqn:phi}, for each $i$,
\begin{align*}
\mu(\Upsilon'_{i}) 
  & = \frac12\theta_{R}(\ell,\ell)\mu(B_{O}(\ell)\setminus B_{O}(\ell-1))
  = (1+o(1))(1-e^{-\alpha})\frac{\nu}{n}e^{(1-\alpha)(R-\ell)}.
% \\
%  & =(e+o(1))(1-e^{-\alpha})\frac{\nu}{n}Re^{-M}.
\end{align*}
Clearly, the events $\layer\cap\Upsilon'_{1}\neq\emptyset,...,
  \layer\cap\Upsilon'_{18}\neq\emptyset$ are independent. 
Hence, by our choice of $\ell$, 
\begin{equation*}\label{evB}
\Pr{(\mathcal{B})} 
  =(1-e^{-\nu(1+o(1))(1-e^{-\alpha})e^{(1-\alpha)(R-\ell)}})^{18}=1+o(1).
\end{equation*}
To prove~\eqref{it:B2}, note that if two vertices in $\layer_{\ell}$ form an 
  angle at the origin of at most $\theta_{R}(\ell,\ell)$, then by 
  Remark~\ref{rem:monotonTheta} they are adjacent.
Thus, every vertex in $\Upsilon'_{i}$ is connected 
  by an edge to every vertex in 
  $\Upsilon'_{i-1}\cup\Upsilon'_{i}\cup\Upsilon'_{i+1}$, 
  since the maximal angle such pairs of vertices form is,
  by our choice of $\phi$, at most 
  $2\frac{\phi}{18}=\theta_{R}(\ell,\ell)$. 
%\dmc{If we agree to change above, also here. but perhaps you don't agree, so i wait}
\end{proof}

Henceforth, for two points $p,p'\in B_{O}(R)$ let $\Delta\phi_{p,p'}$ denote 
  the small angle in $[0,\pi)$ between $p$ and $p'$ formed at the origin.
By definition of $\theta_R(\cdot,\cdot)$, we know that 
  $\dist(p,p')\leq R$ if and only if 
  $\Delta\phi_{p,p'}\leq\theta_R(r_p,r_{p'})$.
Now, for $i\in\{0,\ldots,R-\ell\}$, 
  let $\Upsilon_{\ell+i}$ be the collection of points in 
  $B_{O}(\ell+i)\setminus B_{O}(\ell+i-1)$ that belong to the $(2\upsilon_{\ell+i})$-sector
  with the same bisector as $\Psi$ where
\[
\upsilon_{\ell+i}:=\frac{\phi}{2}+\sum_{j=0}^{i-1}\theta_R(\ell-1+j,\ell+j).
\]
(Note that the previous definition of $\Upsilon_{\ell}$ is consistent
  with the one given before Lemma~\ref{ev:B}.)

Similarly, 
  for $i\in\{0,\ldots,R-\ell\}$, 
  let $\Xi_{\ell+i}$ be the collection of points in 
  $B_{O}(\ell+i)\setminus B_{O}(\ell+i-1)$ that belong to the 
  $(2\xi_{\ell+i})$-sector
  with the same bisector as $\Psi$ where
\[
\xi_{\ell+i}:=\theta_{R}(\ell-1+i,\ell-1+i)+\frac{\phi}{2}+\xi,
\]
and $\displaystyle\xi:=\sum_{j=0}^{R-\ell-1}\theta_R(\ell-1+j,\ell+j)$.

Finally, let $\displaystyle\Xi
     := \bigcup_{i=0}^{R-\ell} \Xi_{\ell+i}$
  and $\displaystyle\Upsilon
     := \bigcup_{i=0}^{R-\ell}\Upsilon_{\ell+i}$
  (see Figure~\ref{fig:Xi}).
Clearly, $\Upsilon\subseteq\Xi$.

\begin{figure}[htbp]
\centering
\begin{tikzpicture}[scale=0.9]
\pgfmathsetmacro{\angXi}{10};
\pgfmathsetmacro{\angIn}{7};
\pgfmathsetmacro{\angOut}{14};
\pgfmathsetmacro{\rout}{15};
\pgfmathsetmacro{\rin}{12};
\node [left] at (0,0) {$O$};
\draw [fill] (0,0) circle (1 pt);

\draw (0,0) -- (-\angOut:\rout);
\draw (0,0) -- (\angOut:\rout);
\draw [very thick] (0,0) ++(-\angOut:\rout) arc (-\angOut:\angOut:\rout);
\draw (0,0) ++(-\angOut:\rin) arc (-\angOut:\angOut:\rin);

\draw [fill=gray!50] (0,0) ++(-13.5:\rin) arc (-13.5:13.5:\rin) -- (13.5:\rin+0.5) arc (13.5:-13.5:\rin+0.5) -- cycle;
\draw [fill=gray!50] (0,0) ++(-11.29:\rin+0.5) arc (-11.29:11.29:\rin+0.5) -- (11.29:\rin+1.0) arc (11.29:-11.29:\rin+1.0) -- cycle;
\draw [fill=gray!50] (0,0) ++(-10.47:\rin+1.0) arc (-10.47:10.47:\rin+1.0) -- (10.47:\rin+1.5) arc (10.47:-10.47:\rin+1.5) -- cycle;
\draw [fill=gray!50] (0,0) ++(-10.17:\rin+1.5) arc (-10.17:10.17:\rin+1.5) -- (10.17:\rin+2.0) arc (10.17:-10.17:\rin+2.0) -- cycle;
\draw [fill=gray!50] (0,0) ++(-10.06:\rin+2.0) arc (-10.06:10.06:\rin+2.0) -- (10.06:\rin+2.5) arc (10.06:-10.06:\rin+2.5) -- cycle;
\draw [fill=gray!50] (0,0) ++(-10.02:\rin+2.5) arc (-10.02:10.02:\rin+2.5) -- (10.02:\rin+3.0) arc (10.02:-10.02:\rin+3.0) -- cycle;
%\draw [fill=gray] (0,0) ++(-\angIn:\rin) arc (-\angIn:\angIn:\rin) -- (\angIn:\rout) arc (\angIn:-\angIn:\rout) -- cycle;

\draw [dashed,gray] (0,0) -- (-\angXi:\rout);
\draw [dashed,gray] (0,0) -- (\angXi:\rout);
\draw [dashed,gray] (0,0) -- (-\angIn:\rout);
\draw [dashed,gray] (0,0) -- (\angIn:\rout);

%\draw [dotted,gray] (0:\rin+1.6) -- (0:\rout-0.6);

% Display angles
\draw [dotted] (-\angXi:\rout) -- (-\angXi:\rout+0.75);
\draw [dotted] (\angXi:\rout) -- (\angXi:\rout+0.75);
\draw [dotted] (-\angIn:\rout) -- (-\angIn:\rout+0.75);
\draw [dotted] (\angIn:\rout) -- (\angIn:\rout+0.75);
\draw [dotted] (-\angOut:\rout) -- (-\angOut:\rout+1.75);
\draw [dotted] (\angOut:\rout) -- (\angOut:\rout+1.75);
\draw [<->] (0,0) ++(-\angIn:\rout+0.75) arc (-\angIn:\angIn:\rout+0.75) node [midway,right] {$\phi$};
\draw [<->] (0,0) ++(-\angOut:\rout+1.75) arc (-\angOut:\angOut:\rout+1.75) node [midway,right] {$2\phi$};
\draw [<->] (0,0) ++(-\angIn:\rout+0.75) arc (-\angIn:-\angXi:\rout+0.75) node [midway,right] {$\xi$};
\draw [<->] (0,0) ++(\angIn:\rout+0.75) arc (\angIn:\angXi:\rout+0.75) node [midway,right] {$\xi$};

% Display radial distances
\draw [dotted] (\angOut+90:0) -- (\angOut+90:2.0);
\draw [dotted] (\angOut:\rout) -- ++(\angOut+90:2.0);
\draw [dotted] (\angOut:\rin) -- ++(\angOut+90:1.0);
\draw [<->] (\angOut+90:1.0) -- ++(\angOut:\rin) node [midway,above] {$\ell-1$};
\draw [<->] (\angOut+90:2.0) -- ++(\angOut:\rout) node [midway,above] {$R$};
\draw [dotted] (-\angOut:\rin) -- ++(-\angOut-90:0.75);
\draw [<->] (-\angOut-90:1.0) ++(-\angOut:\rin) -- ++(-\angOut:0.5) node [midway,below] {$1$};
\draw [<->] (-\angOut-90:1.0) ++(-\angOut:\rin+0.5) -- ++(-\angOut:0.5) node [midway,below] {$1$};
\draw [<->] (-\angOut-90:1.0) ++(-\angOut:\rin+1.0) -- ++(-\angOut:0.5) node [midway,below] {$1$};
\draw [<->] (-\angOut-90:1.0) ++(-\angOut:\rin+1.5) -- ++(-\angOut:0.5) node [midway,below] {$1$};
\draw [<->] (-\angOut-90:1.0) ++(-\angOut:\rin+2.0) -- ++(-\angOut:0.5) node [midway,below] {$1$};
\draw [<->] (-\angOut-90:1.0) ++(-\angOut:\rin+2.5) -- ++(-\angOut:0.5) node [midway,below] {$1$};
\draw [dotted] (-\angOut:\rin+0.5) -- ++(-\angOut-90:1.0);
\draw [dotted] (-\angOut:\rin+1.0) -- ++(-\angOut-90:1.0);
\draw [dotted] (-\angOut:\rin+1.5) -- ++(-\angOut-90:1.0);
\draw [dotted] (-\angOut:\rin+2.0) -- ++(-\angOut-90:1.0);
\draw [dotted] (-\angOut:\rin+2.5) -- ++(-\angOut-90:1.0);
\draw [dotted] (-\angOut:\rin+3.0) -- ++(-\angOut-90:1.0);

\pgfdeclarepatternformonly{ltrdiagonals}%
{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{10pt}{10pt}}%
{\pgfqpoint{9pt}{9pt}}{\pgfsetlinewidth{0.4pt}\pgfpathmoveto{\pgfqpoint{0pt}{0pt}}%
\pgfpathlineto{\pgfqpoint{9.1pt}{9.1pt}}%
\pgfusepath{stroke}}%
\draw[%top color=black!96, bottom color=black!16,
      fill opacity=0.64,
      postaction={fill,pattern=ltrdiagonals,pattern color=black!84}
     ] (0,0) ++(-\angIn:\rin) arc (-\angIn:\angIn:\rin) -- (\angIn:\rin+0.5) arc (\angIn:8.89:\rin+0.5) -- (8.89:\rin+1.0) arc (8.89:9.6:\rin+1.0) -- (9.6:\rin+1.5) arc (9.6:9.85:\rin+1.5) -- (9.85:\rin+2.0) arc (9.85:9.94:\rin+2.0) -- (9.94:\rin+2.5) arc (9.94:9.98:\rin+2.5) -- (9.98:\rout) arc (9.98:-9.98:\rout) -- (-9.98:\rin+2.5) arc (-9.98:-9.94:\rin+2.5) -- (-9.94:\rin+2.0) arc (-9.94:-9.85:\rin+2.0) -- (-9.85:\rin+1.5) arc (-9.85:-9.6:\rin+1.5) -- (-9.6:\rin+1.0) arc (-9.6:-8.89:\rin+1.0) -- (-8.89:\rin+0.5) arc (-8.89:-\angIn:\rin+0.5) -- cycle;

\draw (0,0) ++(-\angOut:\rin+0.0) arc (-\angOut:\angOut:\rin+0.0);
\draw (0,0) ++(-\angOut:\rin+0.5) arc (-\angOut:\angOut:\rin+0.5);
\draw (0,0) ++(-\angOut:\rin+1.0) arc (-\angOut:\angOut:\rin+1.0);
\draw (0,0) ++(-\angOut:\rin+1.5) arc (-\angOut:\angOut:\rin+1.5);
\draw (0,0) ++(-\angOut:\rin+2.0) arc (-\angOut:\angOut:\rin+2.0);
\draw (0,0) ++(-\angOut:\rin+2.5) arc (-\angOut:\angOut:\rin+2.5);
\end{tikzpicture}
\caption{Region $\Xi$ is shown shaded in gray and
  region $\Upsilon$ diagonally hatched (not to scale).}\label{fig:Xi}
%\mkc{I tried re-doing the figure with correct relative scaling between $\phi$, $\upsilon_{\ell+i}$'s and 
%  $\xi_{\ell+i}$'s, but then the differences between the $\upsilon_{\ell+i}$'s and 
%  $\xi_{\ell+i}$'s are impossible to notice. Should we leave it like this? Should we add a comment that 
%  the scaling is not the ``real'' one?}
\end{figure}

Next we establish several facts concerning regions $\Xi$ and $\Upsilon$,
  but first we bound $\xi$ just defined.
By Lemma~\ref{lem:aproxAngle}, 
  the formula for the sum of a geometric series,
  since $R=2\log\frac{n}{\nu}$, and by our choice of $\ell$ 
\begin{equation}\label{eqn:xi}
\xi %= \sum_{j=0}^{R-\ell-1}\theta_R(\ell-1+j,\ell+j)
  = (2+o(1))\frac{\nu}{n}e^{R-\ell+\frac12}\sum_{j=0}^{R-\ell-1}e^{-j}
  = (2+o(1))\frac{e^{3/2}}{e-1}\frac{\nu}{n}e^{R-\ell}.
\end{equation}
Since $e^{3/2}/(e-1)< 3$, by~\eqref{eqn:phi},
  and our choice of $\phi$, for sufficiently large $n$, 
\begin{equation}\label{eqn:phiXi}
%\frac16\phi\leq
\xi < 3\theta_R(\ell,\ell) = \frac{1}{3}\phi. 
\end{equation}

Let $\calC$ be the event that there is no vertex in 
  $\Xi\setminus\Upsilon$.
\begin{lemma}\label{ev:C}
For sufficiently large $n$, the following hold:
\begin{enumerate}[(i).-]
%\item\label{it:propXi1}
%$\Phi'\setminus B_{O}(\ell-1)\subseteq\Upsilon\subseteq \Xi$.
%
\item\label{it:C1}
For some constant $C_0=C_0(\alpha)$ depending only on $\alpha$, the probability that $\calC$ occurs is at least $e^{-C_{0}\nu Re^{-M}}$.

\item\label{it:C2}
If $p\in (B_{O}(R)\setminus B_{O}(\ell-1))\setminus \Xi$ 
  and $p'\in\Upsilon$, then %the distance between $p$ and $p'$ is at least $R$, i.e., 
  $\dist(p,p')> R$.%\dmc{I would eliminate the wording and just say that "then $\dist(p,p') > R$"}
\end{enumerate}
\end{lemma}
\begin{proof}
To prove~\eqref{it:C1}, observe that by  
  Lemma~\ref{lem:aproxAngle}, Corollary~\ref{cor:medidalb},
  by definition of $\Xi_{\ell+i}$, the formula
  for the sum of a geometric series and since $\sqrt{e}/(e-1) < 1$,
%\[
%2\Big((2e+o(1))\frac{\nu}{n}e^{R-\ell-i}
%  +(2\sqrt{e}+o(1))\frac{\nu}{n}e^{R-\ell}\sum_{j=i}^{R-\ell-1}e^{-j}\Big)
%  (1-e^{-\alpha})e^{-\alpha(R-\ell-i)}
%\]
\begin{align*}
\mu(\Xi_{\ell+i}\setminus\Upsilon_{\ell+i}) 
  & 
  = 2(\xi_{\ell+i}-\upsilon_{\ell+i})
      \mu(B_{O}(\ell+i)\setminus B_{O}(\ell-1+i)) \\
  & = 2
  \Big((2e+o(1))\frac{\nu}{n}e^{R-\ell-i}
  +(2\sqrt{e}+o(1))\frac{\nu}{n}e^{R-\ell}\sum_{j=i}^{R-\ell-1}e^{-j}\Big)
  (1-e^{-\alpha})e^{-\alpha(R-\ell-i)} \\
  & \leq  (8e+o(1))(1-e^{-\alpha})\frac{\nu}{n}e^{(1-\alpha)(R-\ell-i)}.
\end{align*}
Hence, again by the formula for the sum of a geometric series and our choice of $\ell$,
\[
\mu(\Xi\setminus\Upsilon)\leq \frac{(8e+o(1))(1-e^{-\alpha})}{1-e^{-(1-\alpha)}}\frac{\nu}{n} e^{(1-\alpha)(R-\ell)}
  (1-e^{-(1-\alpha)(R-\ell)})
  <  C_0\frac{\nu}{n}Re^{-M},
\]
where $C_0$ is a constant depending only on $\alpha$. The sought after lower bound on the probability that 
  $\layer\cap\Xi\setminus\Upsilon$ is empty follows immediately.
  
Next, consider~\eqref{it:C2}.
To prove that $\dist(p,p')>R$ it suffices to show that 
  $\Delta\phi_{p,p'}>\theta_{R}(r_p,r_{p'})$.
Assume $p\in (B_{O}(\ell+i)\setminus B_{O}(\ell+i-1))\setminus\Xi$
  and $p'\in \Upsilon_{\ell+i'}$.
Hence, 
\begin{align*}
\Delta\phi_{p,p'} & >\xi_{\ell+i}-\upsilon_{\ell+i'}
  = \theta_{R}(\ell-1+i,\ell-1+i)+\sum_{j=i'}^{R-\ell-1}\theta_R(\ell-1+j,\ell+j)
\\
  & 
  = (2e+o(1))\frac{\nu}{n}e^{R-\ell}\big(e^{-i}
   + e^{-i'}\frac{\sqrt{e}}{e-1}(1-e^{-(R-\ell-i')})\big),
\end{align*}
where the last equality follows from Lemma~\ref{lem:aproxAngle},
  since $R=2\log\frac{n}{\nu}$, and the formula for the sum of a geometric 
  series.
If $i' < R-\ell$, then $e^{-(R-\ell-i')} \leq e^{-1}$, and 
  since $\sqrt{e}(1-e^{-1})/(e-1)\approx 0.61$, 
  applying Jensen's inequality we obtain that 
  for sufficiently large $n$, %\dmc{removed the term $\frac{\sqrt{e}(1-e^{-1})}{e-1} $ below. If you put the first inequality the second is equality or not? I would put equality}
%\dmc{would put strict inequality below or put a different constant (which we can, since $\sqrt{e}(1-e^{-1})/(e-1)>0.6$) }
\[
\Delta\phi_{p,p'} 
  > (2e+o(1))\frac{\nu}{n}e^{R-\ell}e^{-\frac12(i+i')}= \theta_{R}(\ell-1+i,\ell-1+i').
\]
If $i'=R-\ell$, then $e^{-i} \ge e^{-\frac12(i+i')}$ and $e^{-(R-\ell-i')}=1$, 
  so by Remark~\ref{rem:monotonTheta},
\[
\Delta\phi_{p,p'} >  \theta_{R}(\ell-1+i,\ell-1+i) \ge \theta_{R}(\ell-1+i, \ell-1+i').
\] 
%  so the last stated lower bound on $\Delta\phi_{p,p'}$ still holds.

Now, by Remark~\ref{rem:monotonTheta}, Lemma~\ref{lem:aproxAngle},
  and again since $R=2\log\frac{n}{\nu}$,
\[
\theta_{R}(r_p,r_{p'})\leq\theta_{R}(\ell-1+i,\ell-1+i')
  = (2e+o(1))\frac{\nu}{n}e^{R-\ell}e^{-\frac12(i+i')}.
\]
The last three displayed bounds imply that,
  for a sufficiently large $n$ (independent of $i$ and $i'$), we have 
  $\Delta\phi_{p,p'}> \theta_{R}(r_p,r_{p'})$ as claimed.  
\end{proof}

Observe that $\Xi\setminus\Upsilon$ is the union of two disconnected regions,
  say $\calW'$ and $\calW''$.
We refer to any such region that does not contain vertices as a 
  \emph{wall} 
  (Lemma~\ref{ev:C} part (\ref{it:C2}) corresponds exactly to the 
  second property satisfied by walls as described in Section~\ref{sec:intro}).


For a given $\Psi$, let $H$ be the subgraph of $G$ induced by 
  $V\cap\Upsilon$, where $\Upsilon=\Upsilon(\Psi)$, 
  and denote by $C:=C(\Upsilon)$ the collection of connected components 
  of $H$ that contain at least one vertex in $\layer\cap\Upsilon_\ell$. 
%\dmc{I would put here the defintiion: Let $\calG$ be the event that $C$ contains at least $\Omega((\log n)^{1/(1-\alpha)})$ vertices.}

Let $\calG$ be the event that $C:=C(\Upsilon)$ has size 
  $\Omega((\log n)^{\frac{1}{1-\alpha}})$.
\begin{lemma}\label{ev:G}
The event $\calG$ occurs a.a.s.
Moreover, all area exposed in $\calG$ is inside $\Upsilon$.
\end{lemma}
\begin{proof}
Let $\eta=\eta(\alpha, \nu)$ be a sufficiently large constant, let 
  $\Phi$ be the $\frac{\phi}{3}$-sector 
  with the same 
  bisector as $\Psi$, and let $\ell':=R-\frac{c\log R}{1-\alpha}$ for some 
  small constant $0 < c < 1$. 
For each vertex $z \in\layer_{R-\eta}\cap\Phi$, 
  let $X_z$ be the indicator random variable that indicates 
  whether there exists a path 
  $z=z_{R-\eta},\ldots, z_{\ell'}$ in $G$ so that $z_i\in\layer_{i}$
  for every $i$.

We claim that for a sufficiently large $n$, there is a $\delta>0$ such that if
  $z\in\layer_{R-\eta}\cap\Phi$, then the expected value of $X_z$ is 
  at least $\delta$.
Indeed, suppose that for some $i$ we found a path until $z_{i+1}$. 
By Lemma~\ref{lem:aproxAngle}, Remark~\ref{rem:monotonTheta},
  and Corollary~\ref{cor:medidalb}, 
  the region $\calR\subseteq B_{O}(i)\setminus B_{O}(i-1)$ 
  in which the next  
  vertex $z_{i}$ with the desired properties can be found satisfies
\begin{equation}\label{measureB}
\mu(\calR) 
  \ge \theta_R(i+1,i)\mu(B_{O}(i)\setminus B_{O}(i-1))
  = (2+o(1))(1-e^{-\alpha})\frac{\nu}{n}e^{(1-\alpha)(R-i)-\frac12},
\end{equation}
and hence, with probability at most 
  $e^{-(2+o(1))\nu (1-e^{-\alpha})e^{(1-\alpha)(R-i)-\frac12}}$ no such vertex is found.
Thus, for some positive constant $\delta > 0$, assuming 
  $\eta$ was chosen sufficiently large,
\begin{equation}\label{ev:Pz}
\Ex{X_z}
  \ge 1-\sum_{i=\ell'}^{R-\eta-1} e^{-(2+o(1))\nu (1-e^{-\alpha}) e^{(1-\alpha)(R-i)-\frac12}} 
  \ge \delta.
\end{equation}

Now, let $X:=\sum_{z}X_z$ where the summation is over the $z$'s in
  $\layer_{R-\eta}\cap\Phi$.
We claim that $X=(1+o(1))\Ex{X}$ a.a.s.
Indeed, by Lemma~\ref{lem:aproxAngle}, Corollary~\ref{cor:medidalb},
  and~\eqref{eqn:phi}, 
  we have $\mu(\Phi\cap B_{O}(R-\eta)\setminus B_{O}(R-\eta-1))
  =\Theta(\frac{1}{n}R^{\frac{1}{1-\alpha}})$.
Thus, by Lemma~\ref{lem:Poisson}, for $\eta$ large enough,
  w.e.p., $|\layer_{R-\eta}\cap\Phi|
  =\Theta((\log n)^{\frac{1}{1-\alpha}})$, and hence  by~\eqref{ev:Pz}, 
  $\Ex{X}=\Theta((\log n)^{\frac{1}{1-\alpha}})$. 
Moreover, in case there is a path 
  $z=z_{R-\eta},\ldots, z_{\ell'}$ in $G$ so that $z_i\in\layer_{i}$
  for every $i$, the total angle between 
  $z$ and $z_{\ell'}$ is 
\[
\Delta\phi_{z,z_{\ell'}}
  \leq\sum_{i=\ell'}^{R-\eta-1}\Delta\phi_{z_i,z_{i+1}}
  \leq\sum_{i=\ell'}^{R-\eta-1}\theta_{R}(i-1,i)
  = O\Big(\frac{\nu}{n}e^{R-\ell'}\Big)
  = O\Big(\frac{\nu}{n}R^{\frac{c}{1-\alpha}}\Big)=o(\phi).
\] 
Also, if two such vertices $z, z'\in\layer_{R-\eta}\cap\Phi$ are at an 
  angle $\omega((\log n)^{\frac{c}{1-\alpha}})$, then 
  $X_z$ and $X_{z'}$ are independent. 
Since $c < 1$, most pairs of vertices are at angular distance 
  $\omega((\log n)^{\frac{c}{1-\alpha}})$, and thus 
  $\Ex{(X^2)}=(1+o(1))(\Ex{X})^2$, so by Chebyshev's 
  inequality, a.a.s.~$X=(1+o(1))\Ex{X}$ as claimed.

By the preceding discussion, in order to conclude
  that a.a.s.~$C$ has size 
  $X=(1+o(1))\Ex{X}=\Omega((\log n)^{\frac{1}{1-\alpha}})$ it is enough 
  to show that a.a.s.~the
  following event occurs: for every vertex $z$ in 
  $\layer_{\ell'}\cap\Phi$ there exists a path 
  $z=z_{\ell'}\ldots z_{\ell}$ in $G$ with $z_i\in\layer_{i}$.
Indeed, similar calculations as the ones performed above
  to estimate $|\layer_{R-\eta}\cap\Phi|$ yield that w.e.p.~$|\layer_{\ell'}\cap\Phi|
  =O((\log n)^{\frac{1}{1-\alpha}})$.
By calculations as in~\eqref{measureB} together with a union bound, 
  the desired event does not occur with probability
\begin{align*}
O((\log n)^{\frac{1}{1-\alpha}}e^{-\log^c n})
  +\Pr{\big(|\layer_{\ell'}\cap\Phi|=\omega((\log n)^{\frac{1}{1-\alpha}}\big)} 
= e^{\Theta(\log \log n)-\log^c n}+o(n^{-1})=e^{-\Theta(\log^c n)}.
\end{align*}

Finally, let $z$ be a vertex in $\layer_{R-\eta}\cap\Phi$ for which
  there exists a path $z=z_{R-\eta},\ldots,z_{\ell}$ in 
  $G$ with $z_i\in\layer_i$ for all $i$.
Note that the angle $\Delta\phi_{z,z_{\ell}}$
  between the endvertices $z$ and $z_{\ell}$ 
  of the path satisfies, by Remark~\ref{rem:monotonTheta}, 
\[
\Delta\phi_{z,z_{\ell}}
  \leq\sum_{i=\ell}^{R-\eta-1}\Delta\phi_{z_i,z_{i+1}}
  \leq\sum_{i=\ell}^{R-\eta-1}\theta_{R}(i-1,i)
  \leq\sum_{i=0}^{R-\ell-1}\theta_{R}(\ell-1+i,\ell+i) = \xi.
\]
Thus, by~\eqref{eqn:phiXi}, the total angle between 
  $z$ and $z_{\ell-1}$ is at most $\frac{1}{3}\phi$.
Since $z$ is a vertex in $\Phi$, it lies within an angle of 
  at most $\frac{\phi}{6}$
  of the bisector of $\Psi$.
Thus, all vertices of the $z,...,z_{\ell}$ path are inside $\Phi$, so by construction are also within $\Upsilon$, and hence in 
  establishing that $\calG$ occurs a.a.s.~only 
  $\Upsilon\cap\Phi$ needs to be exposed.
\end{proof}

%If $\mathcal{G}$ and $\mathcal{B}$ hold, then every vertex $z \in \layer_{\ell'} \cap \Phi'' $ is connected by a path to a vertex in $\layer_{\ell} \cap \Phi' $ without having intermediate vertices of this path outside $ \Phi'\setminus (\Phi'_1 \cup \Phi'_{\frac{\varepsilon}{4}R})$: hence, $\mathcal{G}$ is independent of $\calC$.

Now, in order to have a component disconnected from 
  the giant component it is enough that all vertices in $\Upsilon$
  have no neighbors in $B_{O}(R)\setminus\Upsilon$.
By Lemma~\ref{ev:C} Part~\eqref{it:C2}, this happens if
  $V\cap\Xi\setminus\Upsilon$ is empty and no vertex in $\Upsilon$ can
  have a neighbor in $(B_{O}(R)\setminus B_{O}(\ell-1))\setminus\Upsilon$.
However, it could have neighbors in $B_{O}(\ell-1)$.
We next deal with this situation.
First, we show that it is unlikely for such neighbors to fall within
  $B_{O}(\ell-1)\setminus B_{O}((1-\frac{\beta}{2})R)$ and then we deal
  with the possibility of having neighbors in 
  $B_{O}((1-\frac{\beta}{2})R)$
  (recall that $\beta=\beta(M)$ is a sufficiently small constant).

Let $\calH$ be the event that no vertex in $\Upsilon$ has a neighbor in 
  $B_{O}(\ell-1)\setminus B_{O}((1-\frac{\beta}{2})R)$.
\begin{lemma}\label{ev:H}
There is a constant $C_1=C_1(\alpha)$ depending only on $\alpha$
  so that for sufficiently large $n$ the event $\calH$ occurs with
   probability at least $e^{-C_1\nu Re^{-M}}$.
Moreover, all area exposed in $\calH$ is inside 
  $\Psi\cap B_{O}(\ell-1)\setminus B_{O}((1-\frac{\beta}{2})R)$.
\end{lemma}
\begin{proof}
Since by definition $\upsilon_{\ell+i}$ increases with $i$, 
  all vertices in $\Upsilon$ are within an angle 
  $2\upsilon_{R}= 2(\frac{\phi}{2}+\xi)$, so recalling~\eqref{eqn:phiXi}
  also within an angle $2\phi$.
Moreover, by Remark~\ref{rem:monotonTheta}, 
  between two points within distance at most $R$ one of which is 
  in $B_O(j+1)\setminus B_{O}(j)$, $(1-\frac{\beta}{2})R\leq j\leq\ell-2$,
  and the other one in $\Upsilon$ there is an angle at the origin
  of at most $\theta_R(j,\ell-1)$.
Hence, by Lemma~\ref{lem:aproxAngle} and Lemma~\ref{lem:muBall}, and again
  by our choices for $\phi$ and $\ell$, 
  the expected number of neighbors of the vertices in $\Upsilon$ 
  that are inside $B_{O}(\ell-1)\setminus B_{O}((1-\frac{\beta}{2})R)$
  is at most

\begin{align*}
&
n\sum_{j=(1-\frac{\beta}{2})R}^{\ell-2}2(\upsilon_R+\theta_{R}(j,\ell-1))\mu(B_{O}(j+1)\setminus B_{O}(j)) \\
&\qquad \leq 
  2\phi n\mu(B_{O}(\ell))+ 2\sum_{j=(1-\frac{\beta}{2})R}^{\ell-2}\theta_{R}(j,\ell-1)n\mu(B_{O}(j+1))
\\
&\qquad \leq
  18(2+o(1))\nu e^{(1-\alpha)(R-\ell)} + 
  2(2e^{3/2-\alpha}+o(1))\nu e^{\frac12(R-\ell)}\sum_{k\geq R-\ell}e^{-(\alpha-\frac12)k}
  \\
&\qquad \leq 
  C_1\nu Re^{-M},
\end{align*}
where $C_1$ is a constant depending on $\alpha$, but independent of $M$.
The lower bound on $\PP(\calH)$ immediately follows.

To conclude, observe that 
  all area exposed in $\calH$ is inside the $\psi$-sector $\Psi$, as 
  all area exposed lies within an angle of 
  at most $2(\upsilon_{R}+\theta_{R}(\ell-1,(1-\frac{\beta}{2})R))$,
  which by the preceding discussion, Lemma~\ref{lem:aproxAngle}, 
  and our choices of $\psi$, $\phi$, and $\ell$, is at most 
\[
2\phi + 2(2\sqrt{e}+o(1))e^{\frac12(R-\ell-(1-\frac{\beta}{2})R)}
  = \Big(\frac{\nu}{n}\Big)^{1-\frac{\beta}{2}+o(1)}=o(\psi).
\]
\end{proof}
 
If for a sector $\Psi$ the events $\calB, \calC, 
  \calG, \calH$ hold, then we have found a 
  \emph{precomponent} of size $\Theta((\log n)^{\frac{1}{1-\alpha}})$: by 
  $\calG$ and $\calB$, there is a collection of vertices in $\Upsilon$ connected to each other
  (but perhaps not separated from the giant component) of size  $\Theta((\log n)^{\frac{1}{1-\alpha}})$.
All events are independent or positively correlated: the events 
  $\calB$, $\calC$, and $\calH$ are independent because they
  expose disjoint regions of $\Psi\setminus B_{O}((1-\frac{\beta}{2})R)$.
For the same reason, the events $\calC$, $\calG$, and $\calH$ are 
  independent.
The event $\calG$ is positively correlated with $\calB$.
Hence, by combining Lemmata~\ref{ev:B}, \ref{ev:C}, \ref{ev:G} 
  and \ref{ev:H} we get 
\begin{equation}\label{prec}
\Pr{(\calB\cap\calC\cap\calG\cap\calH)} 
  \ge  (1+o(1))e^{-C_0\nu Re^{-M}}e^{-C_1\nu Re^{-M}}
  = e^{-c_M R}
\end{equation}
for some constant $c_M=c_M(\alpha,\nu) > 0$ that can be made as small as 
  desired by choosing $M$ sufficiently large. %\mkc{Is this the only place where we now require $M$ to be large?}\dmc{I checked and I think yes}
%
%for some $\eta > 0$ (this follows from the fact that $1 - 1/(2\alpha) > 0$ and $(1-\alpha)/(2\alpha^2) > 0$).
Hence, for a given sector $\Psi$, the probability to have a precomponent 
  of size $\Theta((\log n)^{\frac{1}{1-\alpha}})$ is at least $e^{-c_M R}$, 
  independent of $\beta$. 
Observe also that all events $\calB$, $\calC$, $\calG$, 
  $\cal{H}$ expose only areas inside 
  $\Psi\setminus B_{O}((1-\frac{\beta}{2})R)$,  and thus the 
  events corresponding to the existence of a precomponent in different 
  $\psi$-sectors are independent.

Now, consider the partition of $B_O(R)$ into $\psi$-sectors 
  $\Psi_1,\ldots, \Psi_{2\pi/\psi}$. 
  By~\eqref{prec}, the probability that there is no $\psi_i$ with a 
  precomponent is therefore at most
\begin{equation}\label{eq:Prec}
(1-e^{-c_M R})^{n^{1-\beta+o(1)}} \le e^{-n^{1-\beta-c_M+o(1)}},
\end{equation}
which tends to $0$ faster than the inverse of any fixed polynomial in $n$, if $c_M$ is chosen small enough so that $1-\beta-c_M > 0$ (such a choice exists, since $c_M$ is independent of $\beta$). Hence, w.e.p.~there exists a $\psi$-sector $\Psi$ that contains a precomponent of size 
  $\Theta((\log n)^{\frac{1}{1-\alpha}})$.

Let $\calS$ be the event that a randomly chosen $\psi$-sector $\Psi$ 
  is such that  
  all vertices in $\Upsilon=\Upsilon(\Psi)$ have no neighbor 
  inside $B_O((1-\frac{\beta}{2})R)$.
\begin{lemma}\label{ev:P}
The event $\calS$ holds a.a.s.
\end{lemma}
\begin{proof}
By Remark~\ref{rem:monotonTheta}, for a vertex in $V\cap\Upsilon$ not to have 
  a neighbor in $\layer_j$, $j\leq (1-\frac{\beta}{2})R$, a
  region of angle at most $\theta_{R}(\ell-1,j-1)=(2e+o(1))e^{\frac12(R-\ell-j)}$ 
  has to be free of vertices. Also, as observed at the beginning of the proof of Lemma~\ref{ev:H}, all vertices inside $\Upsilon$ are within an angle of $2\phi$.
Hence, the region $\calR\subseteq
  B_{O}((1-\frac{\beta}{2})R)$ that needs to be empty in order for $\calS$ to 
  hold satisfies
\begin{align*}
\mu(\calR) & 
  = (2e+o(1))\sum_{j=0}^{(1-\frac{\beta}{2})R}\big(e^{\frac12(R-\ell-j)}+2\phi\big)e^{-\alpha(R-j)} \\
  & =O(R^{\frac{1}{1-\alpha}}e^{-\alpha R+(\alpha-\frac12)(1-\frac{\beta}{2})R})
  =n^{-1-\beta(\alpha-\frac12)+o(1)}.
  \end{align*}
%\dmc{again above in the last line I would not put $\nu$ in the asymptotic notation}
Thus, the expected number of vertices inside $\calR$ is $o(1)$, and by 
  Markov's inequality, the event $\calS$ holds a.a.s. 
\end{proof}
To prove Theorem~\ref{thm:main}, observe now that if in addition to the existence of a precomponent the event $\calS$ holds, then the precomponent inside the randomly chosen $\psi$-sector $\Psi$ forms a connected component separated from the giant component. Since by~\eqref{eq:Prec} w.e.p.~there is a precomponent, by Lemma~\ref{ev:P}, by a union bound,  a.a.s.~there exists a component of size $\Theta((\log n)^{\frac{1}{1-\alpha}})$.
%
%\dmc{Put it here. I don't know whether we should put it before, because one has to check the proof first that this is indeed possible; but up to you}
%
%\medskip
Summarizing, we have established the following:
\begin{proposition}\label{p:LowerBound}
For $\frac12 < \alpha < 1$, a.a.s.~$L_2(G)=\Theta((\log n)^{\frac{1}{1-\alpha}})$.
\end{proposition}
In fact, we have established that for some sufficiently small $\beta'>0$ a.a.s.~there are $\Omega(n^{\beta'})$ components of size $\Theta((\log n)^{\frac{1}{1-\alpha}})$: indeed, the partition of $B_O(R)$ into $\psi$-sectors can be grouped into groups of sectors making for a total angle of $n^{-\beta''}$, where $\beta'' > 0$ is chosen small enough so that~\eqref{eq:Prec} holds in each group, and also small enough, so that a union bound of all events over all groups still holds as well.

Proposition~\ref{p:UpperBound}, Proposition~\ref{p:LowerBound}, and the 
  previous paragraph argument yield Theorem~\ref{thm:main}.
 %  LocalWords:  eqn coshLaw th ne vw subsectors subsector Poissonized
%  LocalWords:  mk drd Chernoff uw uv subgraphs postaction subgraph
%  LocalWords:  ltrdiagonals ev Pz Chebyshev's measureB precomponent
%  LocalWords:  Markov's

